RCCPAC: A parallel relativistic coupled-cluster program for closed-shell and one-valence atoms and ions in FORTRAN

We report the development of a parallel FORTRAN code, RCCPAC, to solve the relativistic coupled-cluster equations for closed-shell and one-valence atoms and ions. The parallelization is implemented through the use of message passing interface, which is suitable for distributed memory computers. The coupled-cluster equations are defined in terms of the reduced matrix elements, and solved iteratively using Jacobi method. The ground and excited states coupled-cluster wave functions obtained from the code could be used to compute different properties of closed-shell and one-valence atom or ion. As an example we compute the ground state correlation energy, attachment energies, $E$1 reduced matrix elements and hyperfine structure constants.

==> rccpac/Makefile <==
include cmplop


LIB    = nlinear.a linear.a ims.a coul.a 6j.a  prop_1v.a 

LDFLAGS=  $(OPT) $(FORM) $(MEMOP) $(DEBUG)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG)
.SUFFIXES: .o .f
FOBJS= rccpac.o core_indx.o  closefl.o  openfl.o ldrivert0_0v.o  findk.o  \
       ldrivert0_1v.o attachement.o correlation.o findlam.o\
       readorb.o init_0v.o init_1v.o normal.o    \
       quad.o readinp.o setgrd.o  setqic.o setup.o  pairsym.o symm.o      \
       virt_indx.o dr.o fact.o    nldrivert0_0v.o \
       nldrivert0_1v.o t0loc.o diis.o  ninej.o rmin3.o rmax3.o tri1.o 

rccpac.x: $(FOBJS) $(LIB)
	$(FC) $(LDFLAGS) -o rccpac.x $(FOBJS) $(LIB)
	
$(FOBJS):orb.h
%o:%f
	$(FC) -c $(FFLAGS) $<

nlinear.a:
	make -C ./nlinear

linear.a: 
	make -C ./linear

ims.a: 
	make -C ./ims

coul.a: 
	make -C ./coulomb

6j.a: 
	make -C ./sixj

prop_1v.a: 
	make -C ./prop_1v

clean: 
	rm -f *.o *.a *.mod *.f90
	cd ./nlinear; rm -f *.o *.mod *.f90; cd ../
	cd ./linear;  rm -f *.o *.mod *.f90; cd ../
	cd ./ims   ;  rm -f *.o *.mod *.f90; cd ../
	cd ./coulomb; rm -f *.o *.mod *.f90; cd ../
	cd ./prop_1v;  rm -f *.o *.mod *.f90; cd ../
	cd ./sixj;      rm -f *.o *.mod *.f90; cd ../


==> rccpac/coulomb/Makefile <==
include ../cmplop


LDFLAGS=  $(OPT) $(FORM) $(MEMOP)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG) -module ../
.SUFFIXES: .o .f
FOBJS= coul_tab.o  rkval.o  symm_coul.o slater.o slater_new.o \
       yzk.o


#
coul.a :  $(FOBJS)
	ar ur coul.a  $(FOBJS)
	ranlib coul.a
	mv coul.a ../coul.a
#

$(FOBJS):
%o:%f
	$(FC) -c $(FFLAGS) $<


==> rccpac/ims/Makefile <==
include ../cmplop

LDFLAGS=  $(OPT) $(FORM) $(MEMOP)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG) -module ../
.SUFFIXES: .o .f
FOBJS= ims_tab.o ims_ppt0.o ims_hht0.o ims_phhpt0.o ims_ppppt0.o \
       ims_hhhht01.o symm_ims.o imsval.o ims_hht1.o ims_ppt1.o ims_tabt1.o \
       ims_hhhht02.o ims_phhht0.o ims_pphpt0.o ims_tab_add.o 
       
#
ims.a:  $(FOBJS)
	ar ur ims.a  $(FOBJS)
	ranlib ims.a
	mv ims.a ../ims.a
#

$(FOBJS):
%o:%f
	$(FC) -c $(FFLAGS) $<


==> rccpac/linear/Makefile <==
include ../cmplop

LIB    = 
LDFLAGS=  $(OPT) $(FORM) $(MEMOP) $(DEBUG)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG) -module ../
.SUFFIXES: .o .f
FOBJS= dhhhht0.o dhht0.o dphpht0.o dhhhht01.o dppppt01.o  \
       dphhht0.o  dphhpt0.o  dpphpt0.o  dppppt0.o dppt0.o   \
       shhpht0.o  shht0.o  shpppt0.o  shpt0.o \
       sphhpt0.o  sphpht0.o  sppt0.o

	
linear.a:  $(FOBJS)
	ar ur linear.a  $(FOBJS)
	ranlib linear.a
	mv linear.a ../linear.a


$(FOBJS):../orb.h
%o:%f
	$(FC) -c $(FFLAGS) $<


==> rccpac/nlinear/Makefile <==
include ../cmplop

LIB    = 
LDFLAGS=  $(OPT) $(FORM) $(MEMOP) $(DEBUG)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG)  -module ../
.SUFFIXES: .o .f
FOBJS= dnhhhht0.o dnphpht0.o dnphhpt0.o dnppppt0.o dnhpppt0.o \
       dnhhpht0.o snhhppt0.o snhpppt0.o snhhpht0.o \
        dnhhhht01.o dnppppt01.o dnphhpt01.o

nlinear.a:  $(FOBJS)
	ar ur nlinear.a  $(FOBJS)
	ranlib nlinear.a
	mv nlinear.a ../nlinear.a
	
$(FOBJS):../orb.h
%o:%f
	$(FC) -c $(FFLAGS) $<


==> rccpac/sixj/Makefile <==
include ../cmplop


LDFLAGS=  $(OPT) $(FORM) $(MEMOP)
FFLAGS=   $(OPT) $(FORM) $(MEMOP) $(DEBUG)
.SUFFIXES: .o .f
FOBJS= arrange.o  max_6j.o  sixj.o  sixj_ret.o  \
       sixj_tab.o  tri6j.o  tridel.o

#
6j :  $(FOBJS)
	ar ur 6j.a arrange.o  max_6j.o  sixj.o  sixj_ret.o  \
               sixj_tab.o     tri6j.o   tridel.o
	ranlib 6j.a
	mv 6j.a ../6j.a
#

$(FOBJS):6j.h
%o:%f
	$(FC) -c $(FFLAGS) $<

clean:
	rm -f *.o

